On Deep Set Learning and the Choice of Aggregations

Recently, it has been shown that many functions on sets can be represented by sum decompositions. These decompositons easily lend themselves to neural approximations, extending the applicability of neural nets to set-valued inputs---Deep Set learning. This work investigates a core component of Deep Set architecture: aggregation functions. We suggest and examine alternatives to commonly used aggregation functions, including learnable recurrent aggregation functions. Empirically, we show that the Deep Set networks are highly sensitive to the choice of aggregation functions: beyond improved performance, we find that learnable aggregations lower hyper-parameter sensitivity and generalize better to out-of-distribution input size.

==> standardheader.tex <==
\usepackage[l2tabu, orthodox]{nag}


% % % % % % % % % %
% MATH
% % % % % % % % % %
\usepackage{amsmath}	% fleqn for left alignment of math blocks (as in classicthesis)
\usepackage{amssymb}


% % % % % % % % % %
% FLOATS, FIGURAES, AND TABLES
% % % % % % % % % %
\usepackage{graphicx} 		% Required for including images
\usepackage{caption}
\captionsetup{font=small} 	% format=hang,
%\usepackage{subfig}
\usepackage{tabularx}
\setlength{\extrarowheight}{3pt} % increase table row height
\usepackage{pbox} 			% for linebreaking in cells
\usepackage{multicol, multirow}
\usepackage{tikz}
\usetikzlibrary{fit,arrows,shapes}
\usetikzlibrary{decorations.pathreplacing}


% % % % % % % % % %
% MISC
% % % % % % % % % %
\usepackage
[
%disable
]{todonotes}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[english]{babel} % hyphenation, special characters, ...
\usepackage{csquotes}		% recommended with babel for quotes
\usepackage{hyperref}       % hyperlinks
\usepackage{cleveref}		% provides \cref for nice in-document refs
\usepackage{url}            % simple URL typesetting
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage
[
activate={true,nocompatibility}, % activate protrusion and expansion
final,						% enable microtype; use "draft" to disable
tracking=true,
kerning=true,
spacing=true,
factor=1100,				% add 10% to the protrusion amount (default: 1000)
stretch=10,					% reduce stretchability (default: 20)
shrink=10					% reduce shrinkability (default: 20)
]
{microtype}
\usepackage{cancel}			% easy cancelling of terms: \cancel{expression}
